Numerical optimization of a prestressed auxetic metamaterial for vibration isolation

We present a numerical study on an enhanced periodic auxetic metamaterial. Rotating squares mechanism allied to precompression induced buckling give these elastic structures exotic properties. The static properties of the reference structure and the enhanced ones are first compared. After numerical analysis to ascertain the differences between several band calculation methods, we demonstrate the effect of precompression issued stress field on the dispersion diagram of the metamaterial. An optimization study is then performed to assess the potential vibration isolation improvement obtained with the new design. As a result, the bandgaps widths and range are found to be greatly increased by the geometric modifications proposed.

==> macrostrans.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{--> macrostrans.tex - Mai 2011 - version 1.6 - kristof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%\RequirePackage[]{color}
%%\RequirePackage{framed,fancybox} %sept. 2009

%\RequirePackage{fancybox} 
%\typeout{fancybox - OK}

\RequirePackage{pgfcore} 
\typeout{pgfcore - OK}

%%%,pgfbaseimage} %%,pgfbaseshapes}
%%\RequirePackage[version=0.65]{pgf}

\usepgfmodule{shapes} 
\typeout{pgf shapes - OK}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%.. Macros / slides
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\renewcommand{\Huge}{\fontsize{28}{28pt}\selectfont \bf}
\renewcommand{\Huge}{\fontsize{25}{1pt}\selectfont \bf}


\newcommand{\dalembertien}[1]{\begin{pspicture}(0,0.5)(6,5)\psframe[framearc=0.3,linecolor=#1,linewidth=0.5](0,0)(5,5)\end{pspicture}}



\definecolor{PantoneRouge}{rgb}{0.686,0.067,0.114}
\definecolor{PantoneFinoGarnet}{rgb}{0.706,0.035,0.220}



\definecolor{blight}{rgb}{0.7,0.65,1}
%\definecolor{blight_ref}{rgb}{0.8,0.85,1}
\definecolor{gris}{rgb}{0.7,0.7,0.7}

%..test / waves05
%%\definecolor{gris}{rgb}{0.2,0.2,0.2} 
%%\definecolor{gris}{rgb}{0.624,0.624,0.624} 

%%\definecolor{cref}{rgb}{0.1,0.1,0.1}
\definecolor{cref}{rgb}{0.3,0.3,0.3}

\definecolor{green1}{rgb}{0.025,0.8,0.025}      %vert Matlab - cb2
\definecolor{green2}{rgb}{0.20,0.65,0.15}       %rem: vert kakifié avec un poil de rouge (0.20)
\definecolor{green3}{rgb}{0.0,0.5,0.0}
\definecolor{green4}{rgb}{0.0,0.3,0.0}
\definecolor{dgreen}{rgb}{0.0,0.35,0.0}
\definecolor{dgreen}{rgb}{0.0,0.392,0.0}

\definecolor{orange1}{cmyk}{0.,0.6,0.8,0}
\definecolor{noir}{rgb}{0.,0.,0.}

\definecolor{violet1}{rgb}{.932,.51,.932}
\definecolor{mmagenta}{rgb}{1,0,1}
\definecolor{dblue}{rgb}{.0,.0,0.545}
\definecolor{dgreen2}{RGB}{44,85,17}	


\definecolor{dblue}{rgb}{0.,0.,0.5}
\definecolor{cblue}{rgb}{0.127,0.206,0.691}

\definecolor{lightskyblue}{rgb}{0.53,0.81,0.98}
\definecolor{mblue}{rgb}{0.,1.,1}
\definecolor{rblue}{rgb}{0.255,0.412,0.882}       %RoyalBlue
\definecolor{mgreen}{rgb}{0.0,0.7,0.0}

%.. charte graphique ECL 2013 !
\definecolor{recl}{rgb}{0.5882,0.0902,0.1804}
\definecolor{gecl}{rgb}{0.6745,0.6745,0.6745}
\definecolor{becl}{rgb}{0.2235,0.4980,0.7725}
\definecolor{oecl}{rgb}{0.8471,0.6196,0.0980}

\definecolor{sblue}{rgb}{0.,0.7.,1}
\definecolor{LightCyan}{rgb}{0.88,1,1}

\newlength{\boite}
\setlength{\boite}{26.5cm}

\fboxsep=7pt

\newcommand{\titreb}[1]
{\begin{center} \shadowbox{\hspace{17pt} \textcolor{blue}{\huge\bf #1} \hspace{15pt}} \end{center}}

\newcommand{\titrer}[1]
{\begin{center} \shadowbox{\hspace{17pt} \textcolor{red}{\huge\bf #1} \hspace{15pt}} \end{center}}

\newcommand{\titre}[1]
{\begin{center} \shadowbox{\hspace{17pt} \huge\bf #1 \hspace{15pt}} \end{center}}

\newcommand{\stitrer}[1]{\vspace*{-0.4cm} \begin{center} \textcolor{red}{\Large #1} \end{center}}

\newcommand{\titrelb}[1]{\shadowbox{\quad \textcolor{blue}{\huge\bf #1} \quad}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%.. from Julien Berland - new title bar - pgf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclarehorizontalshading{ligne}{0.7mm}
  {color(0cm)=(gris); color(\textwidth)=(dblue)}
  
\pgfdeclarehorizontalshading{ligne1}{0.6mm}
  {color(0cm)=(dblue); color(5cm)=(gris)}  

\pgfdeclarehorizontalshading{ligne2}{0.6mm}
  {color(0cm)=(gris); color(0.1cm)=(gris); color(4cm)=(dblue)}  

\pgfdeclarehorizontalshading{ligne3}{0.6mm}
  {color(0cm)=(gris); color(0.1cm)=(gris)}  
  
  
\pgfdeclarehorizontalshading{rainbow}{100bp}{%
  rgb(0bp)=(1,0,0);
  rgb(26bp)=(1,0,0);
  rgb(33bp)=(1,.5,0);
  rgb(40bp)=(1,1,0);
  rgb(47bp)=(0,1,0);
  rgb(54bp)=(0,1,1);
  rgb(61bp)=(0,0,1);
  rgb(68bp)=(1,0,1);
  rgb(75bp)=(.5,0,.5);
  rgb(100bp)=(.5,0,.5)}
\pgfdeclarehorizontalshading{sblues}{100bp}{%
  rgb(0bp)=(0,.7,1);
  rgb(100bp)=(0,.7,1)}
\pgfdeclarehorizontalshading{reds}{100bp}{%
  rgb(0bp)=(1,0,0);
  rgb(100bp)=(1,0,0)}
\pgfdeclarehorizontalshading{rainbow steps}{100bp}{%
  rgb(0bp)=(1,0,0);
  rgb(32.1bp)=(1,0,0);
  rgb(32.1bp)=(1,.5,0);
  rgb(39.2bp)=(1,.5,0);
  rgb(39.2bp)=(1,1,0);
  rgb(46.4bp)=(1,1,0);
  rgb(46.4bp)=(0,1,0);
  rgb(53.5bp)=(0,1,0);
  rgb(53.5bp)=(0,1,1);
  rgb(60.7bp)=(0,1,1);
  rgb(60.7bp)=(0,0,1);
  rgb(67.9bp)=(0,0,1);
  rgb(67.9bp)=(.75,0,.75);
  rgb(100bp)=(.75,0,.75)}


%\newcommand{\titrej}[1]{ 
%  \begin{center}{\color{dblue} \Huge #1} \\[-8mm] 
%    \textcolor{gris}{ \rule{\textwidth}{0.6mm} } 
%  \end{center} \vspace*{-\baselineskip} }

%\newcommand{\titrej}[1]{ 
%  \parbox[]{\textwidth}{\centering \color{dblue} \Huge #1}\\[-1.2ex]
%    \pgfuseshading{ligne}\vspace{-\baselineskip} }

\newcommand{\titrej}[1]{ 
  \centerline{\color{dblue} \Huge #1}   
    \vspace{-2.0ex}\pgfuseshading{ligne} }  %%\vspace{1.5cm} }

\newcommand{\titreo}[1]{ 
  \centerline{\color{orange1} \Huge #1}   
    \vspace{-2.0ex}\pgfuseshading{ligne} }  %%\vspace{1.5cm} }

\newcommand{\titrek}[1]{ 
  \centerline{\color{dblue} \Huge #1}   
    \vspace{-2.0ex}\pgfuseshading{ligne1} }  %%\vspace{1.5cm} }

\newcommand{\fblue}{{\includegraphics[width=0.6cm]{blue-arrow1.eps}}\hskip 1ex}


\definecolor{ctmp1}{rgb}{0.4,0.2,1.0}
\definecolor{ctmp2}{rgb}{0.,0.,0.}


%%\newcommand{\titres}[1]{ 
%%      \hfill{\huge\boldmath $\color{dblue}\llcorner$ \textbf{\color{dblue} #1} $\color{dblue}\urcorner$}\\[-2ex]}

\newcommand{\titres}[1]{ 
      \hfill{\huge\boldmath $\color{cblue}\llcorner$ \textbf{\color{cblue} #1} $\color{cblue}\urcorner$}\\[-2ex]}


\newcommand{\titrec}[1]{ 
      \hfill{\huge\boldmath\textbf{#1}\begin{pspicture}(2ex,2ex)\psframe[fillstyle=solid,fillcolor=recl,linecolor=white,framearc=0.3](0,-0.03ex)(1.3ex,1.3ex)\end{pspicture}}\\[-2ex]}

\newcommand{\titree}[1]{ 
      \hfill{\huge\boldmath $\color{gecl}\llcorner$ \textbf{\color{recl} #1} $\color{gecl}\urcorner$}\\[-2ex]}




%.. points wiki !

\newcommand{\wkb}{\parbox{1.2ex}{\includegraphics[width=1.2ex]{50px-Bullet-blue.eps}}}
\newcommand{\wkv}{\parbox{1.2ex}{\includegraphics[width=1.2ex]{50px-Bullet-green.eps}}}
\newcommand{\wkr}{\parbox{1.2ex}{\includegraphics[width=1.2ex]{50px-Bullet-red.eps}}}
\newcommand{\wkg}{\parbox{1.2ex}{\includegraphics[width=1.2ex]{50px-Bullet-grey.eps}}}
\newcommand{\wky}{\parbox{1.2ex}{\includegraphics[width=1.2ex]{50px-Bullet-ambar.eps}}}


\def\pourmille{\hbox{$\,^0\!/_{00}$}}





%%.. from beamer ! 
\colorlet{bg}{dblue}
\colorlet{parent.bg}{white}

\pgfdeclareradialshading[bg,parent.bg]{bigsphere}{\huge\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(bg!15);
 color(0.1643835ex)=(bg!75);
 color(0.3287671ex)=(bg!70!black);
 color(0.4520547ex)=(bg!50!black);
 color(0.53ex)=(parent.bg)}


%.. pour fixer la taille des points / police courante
\huge

\pgfdeclareradialshading{auxptdblue}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(dblue!15);
 color(0.1643835ex)=(dblue!75);
 color(0.3287671ex)=(dblue!70!black);
 color(0.4520547ex)=(dblue!50!black);
 color(0.53ex)=(white)}

\pgfdeclareradialshading{auxptblue}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(blue!15);
 color(0.1643835ex)=(blue!75);
 color(0.3287671ex)=(blue!70!black);
 color(0.4520547ex)=(blue!50!black);
 color(0.53ex)=(white)}

\pgfdeclareradialshading{auxptred}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(red!15);
 color(0.1643835ex)=(red!75);
 color(0.3287671ex)=(red!70!black);
 color(0.4520547ex)=(red!50!black);
 color(0.53ex)=(white)}

\pgfdeclareradialshading{auxptgreen}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(green!15);
 color(0.1643835ex)=(green!75);
 color(0.3287671ex)=(green!70!black);
 color(0.4520547ex)=(green!50!black);
 color(0.53ex)=(white)}
 
\pgfdeclareradialshading{auxptorange}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(orange1!15);
 color(0.1643835ex)=(orange1!75);
 color(0.3287671ex)=(orange1!70!black);
 color(0.4520547ex)=(orange1!50!black);
 color(0.53ex)=(white)} 

\pgfdeclareradialshading{auxptrblue}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(rblue!15);
 color(0.1643835ex)=(rblue!75);
 color(0.3287671ex)=(rblue!70!black);
 color(0.4520547ex)=(rblue!50!black);
 color(0.53ex)=(white)} 

\pgfdeclareradialshading{auxptrecl}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(recl!15);
 color(0.1643835ex)=(recl!75);
 color(0.3287671ex)=(recl!70!black);
 color(0.4520547ex)=(recl!50!black);
 color(0.53ex)=(white)} 

\newcommand{\ptdblue}{  \parbox{1.2ex}{\pgfuseshading{auxptdblue}} }
\newcommand{\ptblue}{   \parbox{1.2ex}{\pgfuseshading{auxptblue}} }
\newcommand{\ptred}{    \parbox{1.2ex}{\pgfuseshading{auxptred}} }
\newcommand{\ptgreen}{  \parbox{1.2ex}{\pgfuseshading{auxptgreen}} }
\newcommand{\ptorange}{ \parbox{1.2ex}{\pgfuseshading{auxptorange}} }
\newcommand{\ptrblue}{  \parbox{1.2ex}{\pgfuseshading{auxptrblue}} }
\newcommand{\ptrecl}{   \parbox{1.2ex}{\pgfuseshading{auxptrecl}} }



\LARGE

\pgfdeclareradialshading{auxptdblue1}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(dblue!15);
 color(0.1643835ex)=(dblue!75);
 color(0.3287671ex)=(dblue!70!black);
 color(0.4520547ex)=(dblue!50!black);
 color(0.53ex)=(white)}

\pgfdeclareradialshading{auxptred1}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(red!15);
 color(0.1643835ex)=(red!75);
 color(0.3287671ex)=(red!70!black);
 color(0.4520547ex)=(red!50!black);
 color(0.53ex)=(white)}
 
\pgfdeclareradialshading{auxptgreen1}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(green!15);
 color(0.1643835ex)=(green!75);
 color(0.3287671ex)=(green!70!black);
 color(0.4520547ex)=(green!50!black);
 color(0.53ex)=(white)} 

\pgfdeclareradialshading{auxptblue1}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(blue!15);
 color(0.1643835ex)=(blue!75);
 color(0.3287671ex)=(blue!70!black);
 color(0.4520547ex)=(blue!50!black);
 color(0.53ex)=(white)} 

\pgfdeclareradialshading{auxptrblue1}{\pgfpoint{-0.1849315ex}{.2260273ex}}%
{color(0cm)=(rblue!15);
 color(0.1643835ex)=(rblue!75);
 color(0.3287671ex)=(rblue!70!black);
 color(0.4520547ex)=(rblue!50!black);
 color(0.53ex)=(white)} 

\newcommand{\sptdblue}{ \parbox{1.2ex}{\pgfuseshading{auxptdblue1}} }
\newcommand{\sptred}{   \parbox{1.2ex}{\pgfuseshading{auxptred1}} }
\newcommand{\sptgreen}{ \parbox{1.2ex}{\pgfuseshading{auxptgreen1}} }
\newcommand{\sptblue}{ \parbox{1.2ex}{\pgfuseshading{auxptblue1}} }
\newcommand{\sptrblue}{ \parbox{1.2ex}{\pgfuseshading{auxptrblue1}} }
\normalsize


{\LARGE
\pgfdeclareradialshading{optred}{\pgfpoint{-0.15ex}{0.15ex}}
 {color(0ex)=(red!15!white); color(0.09ex)=(red!75!white);
  color(0.18ex)=(red!70!black); color(0.25ex)=(red!50!black); color(0.6ex)=(black)}

\pgfdeclareradialshading{optdblue}{\pgfpoint{-0.15ex}{0.15ex}}
 {color(0ex)=(dblue!15!white); color(0.09ex)=(dblue!75!white);
  color(0.18ex)=(dblue!70!black); color(0.25ex)=(dblue!50!black); color(0.6ex)=(black)}

\pgfdeclareradialshading{optblue}{\pgfpoint{-0.15ex}{0.15ex}}
 {color(0ex)=(blue!15!white); color(0.09ex)=(blue!75!white);
  color(0.18ex)=(blue!70!black); color(0.25ex)=(blue!50!black); color(0.6ex)=(black)}

\pgfdeclareradialshading{optgreen}{\pgfpoint{-0.15ex}{0.15ex}}
 {color(0ex)=(green!15!white); color(0.09ex)=(green!75!white);
  color(0.18ex)=(green!70!black); color(0.25ex)=(green!50!black); color(0.6ex)=(black)}
}

%%\newcommand{\ptblue}{ \parbox{0.7ex}{\pgfuseshading{optblue}} }
%%\newcommand{\ptred}{  \parbox{0.7ex}{\pgfuseshading{optred}} }
%%\newcommand{\ptdblue}{\parbox{0.7ex}{\pgfuseshading{optdblue}} }
%%\newcommand{\ptgreen}{\parbox{0.7ex}{\pgfuseshading{optgreen}} }

\normalsize

\newcommand{\ptrouge}{ \parbox{1.5ex}{\includegraphics[width=0.7cm]{red-bullet-on-white.ps}} }
\newcommand{\ptvert}{  \parbox{1.5ex}{\includegraphics[width=0.6cm]{green-bullet-on-white.ps}} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\def\barregauche{ {\color{blue} \vrule width 2pt} \hspace{10pt}}

\definecolor{shadecolor}{rgb}{0.,0.,0.8}

\newcommand\boitemsg[2]
{\barregauche\begin{minipage}{#1} #2 \end{minipage}}

\newcommand\boitemsgbis[2]
{\barregauche\begin{minipage}{#1}\begin{shaded} #2 \end{shaded}\end{minipage}}






\newcommand{\bptred}{\begin{list}{\hbox{\includegraphics[width=0.7cm]{red-bullet-on-white.ps}}}{}}
\newcommand{\eptred}{\end{list}}

\newcommand{\bptgreen}{\begin{list}{\hbox{\includegraphics[width=0.6cm]{green-bullet-on-white.ps}}}{}}
\newcommand{\eptgreen}{\end{list}}



\typeout{*** macrotrans.tex - OK ***}



%%%%%%%%%%%%%%%%%%
%.. Style francais
%%%%%%%%%%%%%%%%%%
%% style report
% \def\contentsname{T\lowercase{able des mati\`eres}}
% \def\listfigurename{Liste des figures}
% \def\listtablename{Liste des tableaux}
% \def\bibname{R\'ef\'erences}
% \def\indexname{Index}
% \def\figurename{Figure}
% \def\tablename{Tableau}
% \def\chaptername{Chapitre}
% \def\appendixname{Annexe}
% \def\partname{Partie}
% \def\abstractname{R\'esum\'e}

%% Style article
% \def\refname{R\'ef\'erences}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\pagestyle{fancyplain}
%%\plainheadrulewidth=0.4pt
%%\renewcommand{\chaptermark}[1]{\markboth{\thechapter .\ #1}{\thechapter .\ #1}}
%%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
%%\lhead[\fancyplain{\bf\thepage}{\bf\thepage}]{\fancyplain{}{\bf\rightmark}}
%%\rhead[\fancyplain{}{\bf\leftmark}]{\fancyplain{\bf\thepage}{\bf\thepage}}
%%\cfoot{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%.. def. chapitre %%%%%%%%%%%%%%%
%%\makeatletter
%%\def\@makechapterhead#1{%
%%  \vspace*{50\p@}%
%%  {\parindent \z@ \raggedright
%%   \interlinepenalty\@M
%%   \ifnum \c@secnumdepth >\m@ne
%%     \huge \bfseries \thechapter \quad
%%   \fi
%%   \huge \bfseries #1\par\nobreak
%%   \rule{\textwidth}{1mm}
%%   \vskip 40\p@
%%  }}
%%
%%\def\@makeschapterhead#1{%
%%  \vspace*{50\p@}%
%%  {\parindent \z@ \raggedright
%%   \normalfont
%%   \interlinepenalty\@M
%%   \huge \bfseries #1\par\nobreak
%%    \vskip 40\p@
%%  }}
%%\makeatother


